Distilling Text Style Transfer With Self-Explanation From LLMs

Text Style Transfer (TST) seeks to alter the style of text while retaining its core content. Given the constraints of limited parallel datasets for TST, we propose CoTeX, a framework that leverages large language models (LLMs) alongside chain-of-thought (CoT) prompting to facilitate TST. CoTeX distills the complex rewriting and reasoning capabilities of LLMs into more streamlined models capable of working with both non-parallel and parallel data. Through experimentation across four TST datasets, CoTeX is shown to surpass traditional supervised fine-tuning and knowledge distillation methods, particularly in low-resource settings. We conduct a comprehensive evaluation, comparing CoTeX against current unsupervised, supervised, in-context learning (ICL) techniques, and instruction-tuned LLMs. Furthermore, CoTeX distinguishes itself by offering transparent explanations for its style transfer process.

==> table_figure/dataset.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{@{}lccr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Train}} & \multicolumn{1}{c}{\textbf{Validation}} & \multicolumn{1}{c}{\textbf{Test}} \\ \midrule
Formality (F\&R)                         & 51,967                                 & 2,788                                    & 1,332                              \\
Formality (E\&M)                         & 52,597                                 & 2,877                                    & 1,416                              \\
Detoxification                            & 15,795                                 & 3,948                                    & 670                               \\
Shak.-Modern                          & 18,395                                 & 1,218                                    & 1,462                              \\
% Yelp                                 & 20,000                                 & 100                                     & 400                               \\ 
\bottomrule
\end{tabular}
\caption{Text style transfer datasets.}\label{tab:data}
\end{table}

==> table_figure/previous_table.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \centering
% \scriptsize
% \begin{tabular}{@{}llcc@{}}
% \toprule
% \multicolumn{1}{c}{\textbf{}}          & \multicolumn{1}{c}{\textbf{Models}} & \textbf{F\&R} & \textbf{E\&M} \\ \midrule
% \multirow{6}{*}{{Unsup.}} & \citet{li-2018-delete}                     & 42.41        & -            \\
%                                        & \citet{luo-2019-dual}                              & 53.01        & -            \\
%                                       & \citet{he-2020-probabilistic}                                & -            & 23.09        \\
%                                        & \citet{krishna-2020-reformulating}                               & -            & 31.39        \\
%                                        & \citet{xiao-2021-transductive}                                & 60.99        & -            \\
%                                        & CoTex-unsup (ours)                         & 72.05        & 71.70        \\ \midrule
% \multirow{5}{*}{{Sup.}}                & \citet{niu-2018-multitask}                      & 75.35        & 72.01        \\
%                                        & \citet{wang-2019-harnessing}                             & 77.26        & 71.39        \\
%                                        & \citet{liu-2022-semisupervised}                     & 80.32        & 76.87        \\ 
%                                        & SFT T5 (ours)                                 & 77.12        & 73.01        \\
%                                        & CoTex-sup (ours)                          & 77.13        & 74.65        \\ \bottomrule
% \end{tabular}
% \caption{Comparing CoTeX to previous work on formality transfer. Due to the lack of reporting BLEU in the previous unsupervised studies, we take their outputs and compute BLEU using our evaluation scripts. The BLEU of supervised methods are taken from~\citet{liu-2022-semisupervised}.}
% \label{tab:formality_res}
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[h]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \resizebox{0.4\textwidth}{!}{
% \begin{tabular}{@{}lccc@{}}
% \toprule
% \multicolumn{1}{c}{{\color[HTML]{3531FF} \textbf{Unsup.}}} & \textbf{Delete}    & \textbf{ParaGeDi}   & \textbf{CoTex-unsup (ours)} \\ \midrule
%                                                            & 52.08              & 48.89               & 48.53                       \\ \midrule
% \multicolumn{1}{c}{{\color[HTML]{3531FF} \textbf{Sup.}}}   & \textbf{ParaDetox} & \textbf{SFT (ours)} & \textbf{CoTex-sup (ours)}   \\\midrule
%                                                            & 53.98              & 52.88               & 54.79                       \\ \bottomrule
% \end{tabular}
% }
% \caption{Comparing CoTex to previous work on ParaDetox. We take the predictions of Delete, ParaGeDi, and ParaDetox from \citet{logacheva-etal-2022-paradetox} and run with our evaluation pipeline.}
% \label{tab:detoxic_res}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}



% \begin{table}[h]
% \centering
% \scriptsize
% \begin{tabular}{@{}cccc@{}}
% \toprule
% \textbf{Model} & \textbf{DLSM} & \textbf{STRAP} & \textbf{CoTex-unsup} \\ \midrule
%            & 12.85         & 19.96          & 26.79                \\ \bottomrule
% \end{tabular}
% \caption{Comparing to previous work on Shakespeare to modern English dataset. DLSM~\cite{he-2020-probabilistic} and STRAP~\cite{krishna-2020-reformulating} are trained in unsupervised manner.}
% \label{tab:shakespeare_res}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

==> table_figure/supervised_compare.tex <==

% \begin{table}[]
% \tiny
% \centering
% \begin{tabular}{@{}lcc|lc@{}}
% \toprule
% \multicolumn{1}{c}{\textbf{Models}} & \textbf{BLEU}        & \textbf{BLEU}        & \multicolumn{1}{c}{\textbf{Models}}   & \textbf{BLEU}                                \\ \midrule
% \multicolumn{1}{r}{\textbf{Formality}}       & \textbf{F\&R} & \textbf{ E\&M} & \multicolumn{2}{c}{\textbf{Detoxification}}                                               \\ \midrule
% \citet{niu-2018-multitask}*          & 75.35                & 72.01                & \cellcolor[HTML]{d8d8d8}              & \multicolumn{1}{r}{\cellcolor[HTML]{d8d8d8}} \\
% \citet{wang-2019-harnessing}*        & 77.26                & 71.39                & \cellcolor[HTML]{d8d8d8}              & \multicolumn{1}{r}{\cellcolor[HTML]{d8d8d8}} \\
% \citet{liu-2022-semisupervised}     & \textbf{80.32}       & \textbf{76.87}       & \citet{logacheva-etal-2022-paradetox} & 53.98                                        \\
% SFT (Ours)                          & 77.12                & 73.01                & SFT (Ours)                            & 52.88                                        \\
% CoTex-sup  (Ours)                   & 77.13                & 74.65                & CoTex-sup (ours)                    & \textbf{54.79}                               \\ \bottomrule
% \end{tabular}
% \caption{Comparing to previous supervised methods. \textbf{$^*$}: Taken from~\citet{liu-2022-semisupervised}.}\label{tab:supervised_res}
% \end{table}
